Test-Time Fairness and Robustness in Large Language Models

Frontier Large Language Models (LLMs) can be socially discriminatory or sensitive to spurious features of their inputs. Because only well-resourced corporations can train frontier LLMs, we need robust test-time strategies to control such biases. Existing solutions, which instruct the LLM to be fair or robust, rely on the model's implicit understanding of bias. Causality provides a rich formalism through which we can be explicit about our debiasing requirements. Yet, as we show, a naive application of the standard causal debiasing strategy, counterfactual data augmentation, fails under standard assumptions to debias predictions at an individual level at test time. To address this, we develop a stratified notion of debiasing called stratified invariance, which can capture a range of debiasing requirements from population level to individual level through an additional measurement that stratifies the predictions. We present a complete observational test for stratified invariance. Finally, we introduce a data augmentation strategy that guarantees stratified invariance at test time under suitable assumptions, together with a prompting strategy that encourages stratified invariance in LLMs. We show that our prompting strategy, unlike implicit instructions, consistently reduces the bias of frontier LLMs across a suite of synthetic and real-world benchmarks without requiring additional data, finetuning or pre-training.

==> _tabs/semantic_leakage.tex <==

\begin{table}[h]
\centering
\caption{\textbf{OOC considerably improves counterfactual invariance ($\uparrow$) in both gpt-4o-mini and LLAMA-3-70B.} We report the similarity between the outputs when the entire input, including the exogenous noise, is fixed and only $Z$ varies.}
\scalebox{0.75}{
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{@{}l*{10}{c}@{}}
\cmidrule(lr){1-11}
& \multicolumn{5}{c}{\textbf{gpt-4o-mini}} & \multicolumn{5}{c}{\textbf{LLAMA-3-70B}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
$Z$/$Y$ & Animal/ & Animal/ & Movies/ & Food/ & Hobby/ & Animal/ & Animal/ & Movies/ & Food/ & Hobby/ \\
& Food & Work & Work & Work & Accusation & Food & Work & Work & Work & Accusation \\
\cmidrule(lr){1-11}
Default & 0.333 & 0.417 & 0.386 & 0.483 & 0.633 
& 0.344 & 0.527 & 0.291 & 0.456 & 0.520 \\
Unbiased & 0.374 & 0.437 & 0.396 & 0.483 & 0.532
& 0.347 & 0.501 & 0.342 & 0.331 & 0.669 \\
OOC (ours) & \textbf{0.659} & \textbf{0.633} & \textbf{0.629} & \textbf{0.587} & \textbf{1.000}
& \textbf{0.449} & \textbf{0.711} & \textbf{0.358} & \textbf{1.000} & \textbf{0.934} \\
\cmidrule(lr){1-11}
\end{tabular}
} 
\label{tab:semantic}
\end{table}
